Sketches for Time-Dependent Machine Learning

Time series data can be subject to changes in the underlying process that generates them and, because of these changes, models built on old samples can become obsolete or perform poorly. In this work, we present a way to incorporate information about the current data distribution and its evolution across time into machine learning algorithms. Our solution is based on efficiently maintaining statistics, particularly the mean and the variance, of data features at different time resolutions. These data summarisations can be performed over the input attributes, in which case they can then be fed into the model as additional input features, or over latent representations learned by models, such as those of Recurrent Neural Networks. In classification tasks, the proposed techniques can significantly outperform the prediction capabilities of equivalent architectures with no feature / latent summarisations. Furthermore, these modifications do not introduce notable computational and memory overhead when properly adjusted.

==> todo.tex <==
% HOY

- plot de como evolucionan los hidden states respecto al tiempo, con overlay las estimaciones sobre ellos de los sketches.

EH size vs accuracy (utilizando diferentes confguraciones tipo cambiando hidden size o pasando de input solo las estimaciones)

#EHs vs accuracy utilizando diferentes configs de EHs y inputs a linear

EHRNN vs RNN con las mismas configs en los dos (excepto los EHs)
    - Comparando accuracy
    - Comparando training time
    - Comparando memory usage

- Mirar como afecta la dimension de los hidden states a la accuracy y al numero de sketches requeridos.

Accuracy y num parametros comparando EHRNN con RNN cuando el input para esta ultima son los datos con extra features correspondientes a summaries

Memory utility trade-off de hacer crecer eps del EH.

General
- Influencia de eps en running time y accuracy (electricity)
- Cuando sale rentable utilizar los sketches?

- plot comparando val accuracies de cada modelo usando diferentes tipos de estimaciones

----

- Probar con otro tipo de series temporales, otras series temporales del mismo tipo como airlines y arquitecturas

https://archive.ics.uci.edu/ml/datasets/Dodgers+Loop+Sensor

- TODO comparar con prophet de facebook:

https://archive.ics.uci.edu/ml/datasets/Bar+Crawl%3A+Detecting+Heavy+Drinking
https://archive.ics.uci.edu/ml/datasets/Metro+Interstate+Traffic+Volume

- Dibujo EHRNN
